Scalability in Perception for Autonomous Driving: Waymo Open Dataset

The research community has increasing interest in autonomous driving research, despite the resource intensity of obtaining representative real world data. Existing self-driving datasets are limited in the scale and variation of the environments they capture, even though generalization within and between operating regions is crucial to the overall viability of the technology. In an effort to help align the research community's contributions with real-world self-driving problems, we introduce a new large scale, high quality, diverse dataset. Our new dataset consists of 1150 scenes that each span 20 seconds, consisting of well synchronized and calibrated high quality LiDAR and camera data captured across a range of urban and suburban geographies. It is 15x more diverse than the largest camera+LiDAR dataset available based on our proposed diversity metric. We exhaustively annotated this data with 2D (camera image) and 3D (LiDAR) bounding boxes, with consistent identifiers across frames. Finally, we provide strong baselines for 2D as well as 3D detection and tracking tasks. We further study the effects of dataset size and generalization across geographies on 3D detection methods. Find data, code and more up-to-date information at http://www.waymo.com/open.

==> README <==
Copyright 1993 Gilles F. Robert.
You may freely use, modify and/or distribute this file.
This statement added 2008/11/14 by Clea F. Rees on the basis of the email exchange archived at http://lists.debian.org/debian-tex-maint/2008/05/msg00040.html.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A mathematician often needs special symbols to designate sets such as the
integers, the reals etc..

For the time being, the only fonts providing these special symbols have been:
 - the AMS fonts msbm (older version msym), which are intended for use with
Times and aren't truly what a mathematician expects (the stress is on both
stems instead of being on only the left one).
 - Alan Jeffrey's bbold fonts, which are sans-serif ones, with (almost) no
possibility of design variations for, say, a bold variant.
That was all, and in particular nothing for use with Computer Modern.

I was already working at that time on the project of changing the codes of
romanu.mf, romanl.mf and other files to add a 'Blackboard' variant to
Computer Modern.

                YOU HAVE IT ALL THERE !!!

The whole package contains five 'main' files:
 - blbbase.mf (the 'base') contains the supplementary definitions needed
for double stems etc..
 - blbord.mf (the 'driver') is fairly simple and only makes the necessary
calls.
 - blbordu.mf (based on romanu.mf): programs for uppercase letters.
 - blbordl.mf (based on romanl.mf): programs for lowercase letters.
 - blbordsp.mf (based on romand.mf and punct.mf): programs for the digits~1
and~2 and for parentheses and brackets.

There is also a whole lot of parameter files that are (almost) the same as
those provided by DEK.

For most of them, the only differences are
- change 'cmbase' for 'blbbase' on line~2
- change 'generate roman' for 'generate blbord' on last line
- add two extra parameters (interspace# and cap_interspace#).

A LaTeX(2e) package written by Torsten Hilbrich for using these fonts is also 
available nearby, exactly in ctan/macros/latex/contrib/supported/bbm/

I sincerely hope you'll enjoy using these fonts; if you get into problems
while using them, I should be reachable at

 _ _       Gilles F. ROBERT
|          Unit\'e de Math\'ematiques Pures et Appliqu\'ees
|  _ _ _   \'Ecole Normale Sup\'erieure
|   |   |  46, All\'ee d'Italie
|_ _|_ _|  69364 Lyon Cedex (FRANCE)
    |  \
    |   \  e-mail : gfrobert@umpa.ens-lyon.fr

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

